Lifetime-based Optimization for Simulating Quantum Circuits on a New Sunway Supercomputer

High-performance classical simulator for quantum circuits, in particular the tensor network contraction algorithm, has become an important tool for the validation of noisy quantum computing. In order to address the memory limitations, the slicing technique is used to reduce the tensor dimensions, but it could also lead to additional computation overhead that greatly slows down the overall performance. This paper proposes novel lifetime-based methods to reduce the slicing overhead and improve the computing efficiency, including an interpretation method to deal with slicing overhead, an in-place slicing strategy to find the smallest slicing set and an adaptive tensor network contraction path refiner customized for Sunway architecture. Experiments show that in most cases the slicing overhead with our in-place slicing strategy would be less than the cotengra, which is the most used graph path optimization software at present. Finally, the resulting simulation time is reduced to 96.1s for the Sycamore quantum processor RQC, with a sustainable single-precision performance of 308.6Pflops using over 41M cores to generate 1M correlated samples, which is more than 5 times performance improvement compared to 60.4 Pflops in 2021 Gordon Bell Prize work.

==> author.tex <==
\newcommand{\SDU}{{Shandong University}\xspace}
\newcommand{\TU}{{Tsinghua University}\xspace}
\settopmatter{authorsperrow=1}
% \author[1]{A. Author}
% \author[2]{B. Author}
% \author[4]{C.  Author}
% %\author[2]{Corresponding Author\thanks{email@2nduniversity.com}}
% \affil[1,2]{Institution of the Authors from  University}
% \affil[4]{Institution of the Authors from  College}
% \affil[1]{Email id: aa@gmail.com}
% \affil[2]{Email id: ba@gmail.com}
% \affil[1,4]{Email id: ca@gmail.com}
\newcommand{\tsc}[1]{\textsuperscript{#1}}
\author{Yaojian Chen\tsc{1,2},Yong  Liu\tsc{2,5}, Xinmin Shi\tsc{3},Jiawei Song\tsc{2}, Xin Liu\tsc{2,5}}
%\author{Haohuan Fu\tsc{1,3},Jiawei Song\tsc{1,3}, Pengpeng Zhao\tsc{1,3}, Zhen Wang\tsc{1,3}, Dajia Peng\tsc{2}, Huarong Chen\tsc{1,3}}
\author{ Lin Gan\tsc{1,2},Chu Guo\tsc{4},Haohuan Fu\tsc{1,2},Dexun Chen\tsc{1,2},Guangwen Yang\tsc{1,2}}
\affiliation{
  \institution{\vskip .2cm}
  \institution{1.Tsinghua University, Beijing, China}
  \institution{2.National Supercomputing Center in Wuxi, Wuxi, China  }
  \institution{3.Information Engineering University, Zhengzhou, China}
  \institution{4.Shanghai Research Center for Quantum Sciences, Shanghai, China}
   \institution{5.Zhejiang Lab, Hangzhou, China}
  \country{}
}
%6666666666666
% \author{Yuxuan Li}
% \author{Zhao Liu}
% \author{Lin Gan}
% \author{Haohuan Fu}
% \author{Wei Xue}
% \author{Guangwen Yang}
% \affiliation{
% \institution{Tsinghua University}
% \institution{National Supercomputer Center in Wuxi}
% }

% \author{Qi Shao}
% \author{Mingshan Shao}
% \author{JinXiao Zhang}
% \affiliation{
% \institution{Shandong University}
% }

\renewcommand{\shortauthors}{Yaojian Chen et al.}


%\author{\IEEEauthorblockN{}
%\IEEEauthorblockA{\textit{Department of Computer Science and Technology,} \\
%\textit{Tsinghua University,}\\
%Beijing, China \\
%yj-chen21@mails.tsinghua.edu.cn}
%\and
%\IEEEauthorblockN{ Yong Liu}
%\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
%\textit{name of organization (of Aff.)}\\
%City, Country \\
%email address or ORCID}
%\and
%\IEEEauthorblockN{ Xinmin Shi}
%\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
%\textit{name of organization (of Aff.)}\\
%City, Country \\
%email address or ORCID}
%\and
%\IEEEauthorblockN{ Jiawei Song}
%\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
%\textit{name of organization (of Aff.)}\\
%City, Country \\
%email address or ORCID}
%\and
%\IEEEauthorblockN{ Lin Gan}
%\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
%\textit{name of organization (of Aff.)}\\
%City, Country \\
%email address or ORCID}
%\and
%\\IEEEauthorblockN{ Xin Liu}
%\\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
%\\textit{name of organization (of Aff.)}\\
%\City, Country \\
%\email address or ORCID}
%\\and
%\\IEEEauthorblockN{Haohuan Fu}
%\\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
%\\textit{name of organization (of Aff.)}\\
%\City, Country \\
%\email address or ORCID}
%\\and
%\\IEEEauthorblockN{Guangwen Yang}
%\\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
%\\textit{name of organization (of Aff.)}\\
%\City, Country \\
%\email address or ORCID}
%\\and
%\\IEEEauthorblockN{Dexun Chen}
%\\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
%\\textit{name of organization (of Aff.)}\\
%\City, Country \\
%\email address or ORCID}
%\}


==> ref.tex <==
\begin{thebibliography}{50}
\bibitem{sc17-half-petabyte-simulation-45qubit}
Thomas Haner and Damian S Steiger, \emph{0.5 petabyte simulation of a 45-qubit quantum circuit}, In Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis, SC ’17, pages 33:1–33:10, New York, NY, USA, 2017. ACM.
\bibitem{article2}
Edwin Pednault, John Gunnels, Giacomo Nannicini, Lior Horesh, Thomas Magerlein, Edgar Solomonik, and Robert Wisnieff. \emph{Breaking the 49-qubit barrier in the simulation of quantum circuits}, arXiv:1710.05867,  2017.
\bibitem{article3}
R. Li, B. Wu, M. Ying, X. Sun, and G. Yang. \emph{Quantum supremacy circuit simulation on sunway taihulight}, arXiv preprint arXiv:1804.04797, 2018
\bibitem{article4}
De Raedt, H., et al. \emph{Massively parallel quantum computer simulator, eleven years later}, Computer Physics Communications 237, 47 (2019).
\bibitem{article5}
S. Boixo, S. V. Isakov, V. N. Smelyanskiy, and H. Neven. \emph{Simulation of low-depth quantum circuits as complex undirected graphical models}, arXiv:1712.05384(2017). 
\bibitem{article6}
Markov, I. L. and Shi, Y. \emph{Simulating quantum computation by contracting tensor
networks}, SIAM J. Comput. 38, 963 (2008).
\bibitem{article7}
Bravyi, S. and Gosset, D. \emph{Improved classical simulation of quantum circuits dominated by Clifford gates}, Phys. Rev. Lett. 116, 250501 (2016).
\bibitem{article8}
Z. Y. Chen, Q. Zhou, C. Xue, X. Yang, G. C. Guo, and G. P. Guo, \emph{64-Qubit Quantum Circuit Simulation}, Science Bulletin, vol. 63, pp. 964–971, aug 2018.ACM
\bibitem{article9}
J.~Chen, F.~Zhang, C.~Huang, M.~Newman and Y.~Shi, \emph{Classical simulation of intermediate-size quantum circuits}, arXiv:1805.01450 (2018).
\bibitem{article10}
Chen, M.-C., et al. \emph{Quantum teleportation-inspired algorithm for sampling large random quantum circuits}, arXiv:1901.05003 (2019).
\bibitem{article11}
Guo, C., et al. \emph{General-purpose quantum circuit simulator with Projected Entangled-Pair States and the quantum supremacy frontier}, arXiv:1905.08394 (2019)
\bibitem{article12}
Haohuan Fu, Junfeng Liao, Jinzhe Yang, Lanning Wang,Zhenya Song, Xiaomeng Huang, Chao Yang, WeiXue, Fangfang Liu, Fangli Qiao, Wei Zhao, Xunqiang Yin, Chaofeng Hou, Chenglong Zhang, Wei Ge, Jian Zhang, Yangang Wang, Chunbo Zhou, and Guangwen Yang. \emph{The sunway taihulight supercomputer: system and applications}, Science China Information Sciences,59(7):072001, Jun 2016.
\bibitem{article13}
K. De Raedt, K. Michielsen, H. De Raedt, B. Trieu, G. Arnold,M. Richter, T. Lippert, H. Watanabe, and N. Ito, \emph{Massively parallel quantum computer simulator}, Computer Physics Communications, vol. 176, pp. 121–136, jan 2007.
\bibitem{article14}
M. Smelyanskiy, N. P. D. Sawaya, and A. Aspuru-Guzik, \emph{qHiP-STER: The Quantum High Performance Software Testing Environment},arXiv:1601.07195, 2016.
\bibitem{article15}
H. De Raedt, F. Jin, D. Willsch, M. Nocon, N. Yoshioka, N. Ito, S. Yuan,and K. Michielsen, \emph{Massively parallel quantum computer simulator,eleven years later}, arXiv:1805.04708, 2018.
\bibitem{article16}
D. Gottesman, \emph{The heisenberg representation of quantum computers}, arXiv preprint quant-ph/9807006, 1998.
\bibitem{article17}
S. Aaronson and D. Gottesman, \emph{Improved simulation of stabilizer circuits}, Physical Review A, vol. 70, no. 5, p. 052328, 2004.
\bibitem{article18}
S. Bravyi and D. Gosset, \emph{Improved Classical Simulation of Quantum Circuits Dominated by Clifford Gates}, Physical Review Letters,vol. 116, p. 250501, jun 2016.
\bibitem{article19}
R. S. Bennink, E. M. Ferragut, T. S. Humble, J. A. Laska, J. J. Nutaro,M. G. Pleszkoch, and R. C. Pooser, \emph{Unbiased simulation of near-clifford quantum circuits}, Physical Review A, vol. 95, no. 6, p. 062337, 2017.
\bibitem{article20}
S. Boixo, S. V. Isakov, V. N. Smelyanskiy, R. Babbush, N. Ding,Z. Jiang, M. J. Bremner, J. M. Martinis, and H. Neven, \emph{Characterizing quantum supremacy in near-term devices}, Nature Physics, vol. 14,pp. 1–6, jun 2018.
\bibitem{article21}
I. L. Markov and Y. Shi, \emph{Simulating quantum computation by contracting tensor networks}, SIAM Journal on Computing, vol. 38, pp. 963–981,jan 2008.
\bibitem{article22}
J. Biamonte and V. Bergholm, \emph{Tensor networks in a nutshell}, arXiv preprint arXiv:1708.00006, 2017.
\bibitem{article23}
A. McCaskey, E. Dumitrescu, M. Chen, D. Lyakh, and T. Humble, \emph{Validating quantum-classical programming models with tensor network simulations}, PLOS ONE, vol. 13, pp. 1–19, 12 2018.
\bibitem{article24}
S. Boixo, S. V. Isakov, V. N. Smelyanskiy, and H. Neven, \emph{Simulation of low-depth quantum circuits as complex undirected graphical models}, arXiv:1712.05384 [quant-ph], dec 2017.
\bibitem{article25}
S. Boixo and C. Neill, \emph{The question of quantum supremacy}, Google AI Blog, May 2018. Available on GitHub at https://github.com/sboixo/GRCS.
\bibitem{article26}
J. Chen, F. Zhang, C. Huang, M. Newman, and Y. Shi, \emph{Classical Simulation of Intermediate-Size Quantum Circuits}, arXiv:1805.01450 [quant-ph], may 2018.
\bibitem{article27}
I. L. Markov, A. Fatima, S. V. Isakov, and S. Boixo, \emph{Quantum Supremacy Is Both Closer and Farther than It Appears}, arXiv:1807.10749 [quant-ph], jul 2018.
\bibitem{article28}
B. Villalonga, S. Boixo, B. Nelson, C. Henze, E. Rieffel, R. Biswas, andS. Mandrà, \emph{A flexible high-performance simulator for the verification and benchmarking of quantum circuits implemented on real hardware}, arXiv preprint arXiv:1811.09599, 2018.
\bibitem{article29}
M.-C. Chen, R. Li, L. Gan, X. Zhu, G. Yang, C.-Y. Lu, and J.-W. Pan, \emph{Quantum Teleportation-Inspired Algorithm for Sampling Large Random Quantum Circuits}, arXiv:1901.05003 [quant-ph], January 2019.
\bibitem{article30}
Markov, I. L. and Shi, Y. \emph{Simulating quantum computation by contracting tensor networks}, SIAM J. Comput. 38, 963 (2008).
\bibitem{article31}
S.~Boixo, S. V.~Isakov, V.~N.~Smelyanskiy and H.~Neven,  \emph{Simulation of low-depth quantum circuits as complex undirected graphical models}, arXiv:1712.05384 (2017).
\bibitem{article32}
Guo, C.,Zhao YW,Huang HL. \emph{Verifying Random Quantum Circuits with Arbitrary Geometry Using Tensor Network States Algorithm}, arXiv:2011.02621 (2020)
\bibitem{article33}
Pednault, E., Gunnels, J.A., Nannicini, G., Horesh, L., Magerlein, T., Solomonik, E., Draeger, E., Holland, E.,  Wisnieff, R. \emph{Pareto-Efficient Quantum Circuit Simulation Using Tensor Contraction Deferral}, arXiv: Quantum Physics. (2017).
\bibitem{article34}
Wu, X., Di, S., Dasgupta, E.M., Cappello, F., Finkel, H., Alexeev, Y., Chong, F. (2019). \emph{Full-state quantum circuit simulation by using data compression}, Proceedings of the International Conference for High Performance Computing, Networking, Storage and Analysis.
\bibitem{article35}
Villalonga, B., Lyakh, D., Boixo, S., Neven, H., Humble, T., Biswas, R., Rieffel, E., Ho, A., Mandrà, S. \emph{Establishing the Quantum Supremacy Frontier with a 281 Pflop/s Simulation}, arXiv: abs/1905.00444. (2019).
\end{thebibliography}
